Diagnosing Rarity in Human-Object Interaction Detection

Human-object interaction (HOI) detection is a core task in computer vision. The goal is to localize all human-object pairs and recognize their interactions. An interaction defined by a <verb, noun> tuple leads to a long-tailed visual recognition challenge since many combinations are rarely represented. The performance of the proposed models is limited especially for the tail categories, but little has been done to understand the reason. To that end, in this paper, we propose to diagnose rarity in HOI detection. We propose a three-step strategy, namely Detection, Identification and Recognition where we carefully analyse the limiting factors by studying state-of-the-art models. Our findings indicate that detection and identification steps are altered by the interaction signals like occlusion and relative location, as a result limiting the recognition accuracy.

==> Diagnosing Human-object Interaction Detection/0-introduction.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Three Styles of Opening Sentences
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1. Straight forward, what we do
% This paper strives for / The goal of this paper is recognizing human activities in minutes-long videos. On one hand, current 3D CNNs can learn temporal concepts. But they can model few seconds or up a minute long activities [?, ?]. On the other hand, statistical pooling can aggregate temporal signals over very long videos, but at the cost of neglecting the temporal patterns. To address this problem, we propose to use undirected graphs as a representation for minutes-long human activities.

% 2. Method first
% Undirected graphs are successful in aggregating signal over time [?] and representing its temporal structure [?]. This paper proposed a graph-based representation method to recognize human activities in minutes-long videos.

% 3. Problem first
% Human activities in videos can take many minutes to unfold, each is packed with plentiful of fine-grained visual details. Take for example two activities: “Making a Pancake” or “Preparing Scrambled Eggs”. The question is what makes a difference between these activities? Is it the fine-grained details in each, or the overall painted picture by each? Or both?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ONLY SIMPLY TENSE THROUGHOUT THE PAPER MANUSCRIPT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 0.0 Teaser Figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1.0 Intro sentence, create audience, invite readers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2.0 Problem Definition
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3.0 Related Works
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 5.0 Solution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 6.0 Novelties and Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}


\noindent The goal of HOI detection is to detect all possible human-object pairs and recognize their interactions from an image. It is a core task in computer vision with many applications in robotics~\cite{katz2008manipulating}. A HOI is defined by a triplet of \texttt{<human, interaction, object>}, where the human and the object is a bounding box and the interaction is a \texttt{<verb, noun>} pair, such as \texttt{<ride, bicycle>}. The task received an increasing amount of attention in recent years~\cite{gkioxari2018detecting,qi2018learning,gao2018ican,xu2019learning,peyre2018detecting,gupta2018no,bansal2019detecting,wang2019deep,chafik2020classifying} thanks to the benchmark dataset HICO-Det~\cite{chao2018learning}. The distribution of the training samples for interactions follows a long-tailed distribution where many interactions have few examples, see Figure~\ref{fig:teaser}. Despite the progress in the performance of many-shot interactions, recognizing rare interactions remains a challenge.  

%Going from an input image to HOI detections happens in three consecutive steps, see Figure~\ref{fig:steps}. \textbf{First}, the HOI detector initially localizes all possible humans and objects from the image. Detecting humans and objects of an interaction is challenging since the interaction leads to transformations on the human-object body: the human and the object is occluded by each other, and many interacted objects exhibit a small-area within the image. \textbf{Second}, the HOI detector identifies the real interacting pairs of humans and objects. Among all possible humans and objects, only few is in a real interaction. This step adds to the challenge since many times the signs of an interaction is subtle: In relative locations of human-objects, in the gaze of the human or in the handlebar of the object. \textbf{Third}, the HOI detector needs to determine the interaction predicate for the interacting pairs of humans and objects. This step is challenged by the fact that the HOI detector only has access to few examples for many interaction categories, making it hard to learn fine-grained signs of an interaction category.  

HOI Detection is accomplished in three steps, see Figure~\ref{fig:steps}. \textbf{1. Human-object detection}: HOI detector initially localizes all possible human-objects from the image. This step is challenged by the fact that interactions transform the human-object appearance, such as occlusions due to grasping, making it hard to localize all human-objects. \textbf{2. HOI Identification}: Given the exhaustive pairing of all detected humans and objects, the HOI detector needs to identify the real interacting pairs. In the case of Figure~\ref{fig:steps}, only the rider, and the cow are in an interaction. This step is challenging since the cues of an interacting pair is in their subtlety, such as the relative locations of human-objects, human gaze or object parts. \textbf{3. HOI Recognition}: In this step, HOI detector needs to classify the interaction type of the human-object pair(s), such as \texttt{<hold, cow>} and \texttt{<sit on, cow>} in Figure~\ref{fig:steps}. It is hard to distinguish among many interaction types since only a few examples are available for many interactions. 

%\begin{figure}[t]
  %\dummyfig{Teaser Figure} 
  %\caption{Human-object interactions exhibit a long-tailed distribution. Here is an example of the %distribution of the interaction \textbf{riding} over different object instances.}
%  \label{fig:dummy}
%\end{figure}


\begin{figure}[t]
\begin{center}

\includegraphics[width=0.9\linewidth]{figures/teaser.pdf}
\end{center}
  \caption{Human-object interactions exhibit a long-tail. For example, riding skateboard has more than $1k$ training instances whereas cow, giraffe or sheep only has $1$ example.}
  \label{fig:teaser}
\end{figure}

\begin{figure*}[h]
\includegraphics[width=1.0\linewidth]{figures/stepshoi.pdf}
  \caption{Steps of our diagnostic study. Detection (left), Identification (middle) and Recognition (right).}
  \label{fig:steps}
\end{figure*}


%Proposed techniques highlight the difficulty of recognizing rare HOIs by reporting the recognition performance on both rare and nonrare splits of the testing set~\cite{X}. However, what makes rare interactions particularly challenging? Are human-objects harder to detect? Or HOI identification is particularly hard? In this paper our goal is to answer these questions. We take a step back from engineering a new model, and try to understand the rare interactions with the help of 3 state-of-the-art HOI detectors~\cite{X,X,X} on the well established benchmark of HICO-DET~\cite{X}. We investigate the three steps of HOI detection, with a particular attention to rare categories. Specifically, we try to illuminate the effect of the human-object detection and HOI identification steps on the recognition accuracy for rare interaction categories. 

Existing models highlight the difficulty in recognizing rare HOIs by reporting the performance on both the rare and nonrare (\ie many shots) splits on the benchmark dataset~\cite{chao2018learning}. However, it is not known what makes rare interactions particularly challenging aside from the low number of examples. Are the human-objects of rare interactions harder to detect? Or rare interacting pairs are harder to identify? The goal of our paper is to answer these questions. Instead of engineering a new model, we try to understand the detectability and identifiability of rare interactions with the help of the state-of-the-art HOI detectors~\cite{gao2018ican,chao2018learning,li2019transferable}. 

Our findings are: (i) Localizing human-objects of rare interactions is not challenging, however, detection is altered by the small and occluded human-objects, (ii) Identifying the rare HOIs is challenging and is altered by the background clutter and human-object distance, and (iii) Recognizing rare interactions is influenced by the detection and identification errors, leaving a big room for improvement. 

%\noindent HOI Detection is a core task in computer vision where the goal is to detect all possible human-object pairs from the input and classify their interactions. An interaction is in the form of a \texttt{<verb, noun>} pair such as \texttt{<ride, bicycle>} or \texttt{<eat, cake>}. 
%HOI detection is critical for tasks such as visual imitation learning in robotics~\cite{X} or self-driving cars. Therefore it received an increasing amount of attention in recent years~\cite{XXX} thanks to the availability of big benchmark dataset HICO-Det~\cite{X}. However, the challenge of the task remains as the progress in recent years have been limited. 

%The challenge of HOI detection is many-fold. Even before the final recognition step, the models need to perform two important tasks. First, a HOI detector needs to localize all possible humans and objects in the image. Existing techniques resort to an off-the-shelf detector~\cite{X} for this step. However, an interaction leads to many transformations on the human and object appearance, such as occlusions and deformations which are known to challenge the detection. Secondly, a HOI detector needs to identify, amongst all possible human and object detections, which pair(s) are in an interaction. By doing this, HOI detector ensures that, amongst all possible human-object proposals, only the interacting ones make it to the classification stage, suppressing non-interacting ones. Many times the cues for an interaction is hidden in the subtlety: relative location of human-objects, hand pose or the gaze of the human, or an occluded (invisible) part of an object. It is hard for current Convolutional Neural Networks to reason about such fine-grained visual details within the input. 

%Finally, a HOI detector needs to recognize the type of the interaction for each interacting pairs of human-objects. To learn to distinguish between different types of categories, CNNs need sufficient amount of training examples. However HOIs have a long-tailed distribution where many \texttt{<verb, noun>} combinations are rare, therefore making the recognition difficult. 

%The goal of this work is to diagnose HOI detectors. We take a step back from engineering a new model, and rather try to understand the limitations of existing state-of-the-art HOI detectors~\cite{XXXX}. The outcome of such diagnostic study has proven to be beneficial for many tasks in computer vision such as in object detection~\cite{X}, temporal localization~\cite{X} or multi-human pose estimation~\cite{X}. Such studies go beyond single scalar-based evaluation and investigate the factors that affect the accuracy. HOI detection is not an exception since the contribution of the human-object detection and interaction identification steps is mostly ignored in prior work. To that end, our work develops a three-stage evaluation strategy to take a closer look at existing models. 

%We first investigate the Detectability of Humans and Objects. Specifically, we explore the sensitivity of the off-the-shelf detector to the varying size of humans and objects and their occlusion. Then, we proceed to investigate the Identifiability of Human-Object Interactions. Specifically, we explore how well the existing models can distinguish interacting pairs from non-interacting ones, with the varying size of human-objects and background clutter. Finally, we focus on the Recognizability of Human-Object Interactions. Specifically we investigate how do the existing techniques perform with the changes in human-object area, background clutter, and the errors caused by human-object detection and identification steps. 

%Our contributions are as follows: \textit{i).} We propose to diagnose HOI detectors in three controlled steps, \textit{ii).} We show that models are challenged by the detection and the identification of humans, objects and their identification, \textit{iii).} We show that there is a strong connection between recognition and human-object detection and identification, suggesting further research into this direction. 



==> Diagnosing Human-object Interaction Detection/2-method.tex <==




\section{Empirical Material}



%In this part we first describe Human-object interaction detection models evaluated in this work. Then, we describe our analysis methodology before presenting experiments. 

\subsection{Benchmark Dataset}

For our analysis, we resort to HICO-Det dataset~\cite{chao2018learning}. HICO-Det is the biggest HOI detection benchmark, with a diverse set of categories. The dataset comes with (i) Human-object bounding boxes for detection, (ii) Human-object interaction pair annotations for identification, and (iii) Human-object interaction types for recognition. A typical human-object concurrently performs multiple interactions such as holding, sitting on and riding a bicycle which is exhaustively annotated. The dataset has in total $47k$ number of images, with more than $150k$ human-object pair annotations. There exists $600$ distinct interaction types of which $168$ are rare, for $80$ unique nouns and $117$ unique verbs. %Among $600$ interactions, $168$ have less than $10$ training examples, and falls into the rare split in the dataset. 

A unique property of the dataset is, for each noun in the dataset, there exists a no-interaction category, where at least a human and the target object is in the image, though not performing an interaction(\eg the man and the car in Figure~\ref{fig:steps}). This enforces the models to focus on the interaction characteristics as opposed to leveraging human-object co-occurrence. 

\subsection{Benchmark HOI Detectors}

For our diagnostic purposes, we resort to three state-of-the-art HOI detectors, namely HO-RCNN~\cite{chao2018learning}, iCAN~\cite{gao2018ican}, and TIN~\cite{li2019transferable} for the following reasons: (i) Their high performance, (ii) Standard use of the same object detector, the same backbone and the same number of layers and (iii) Publicly available code. Here, we present an overview.

%\partitle{HO-RCNN~\cite{chao2018learning}.} HO-RCNN is a three-streams Convolutional Neural Network (CNN) where each stream takes as input the human, the object and their pairwise location layout. Human and object streams are fed with local representations of the corresponding human and object detections, obtained via Region-of-Interest (ROI) pooling. The model makes use of Faster-RCNN as backbone architecture, and also relies on this detector for initial localization of human and object regions. Pairwise stream takes as input a a canvas with two layers where each layer encodes the human and object bounding box locations respectively. The goal is to take advantage of the global representation of the human, the object and their relative location which could be useful in identifying their interaction if it exists. Final prediction for HOIs is done via combination of the individual predictions of these three streams. This model yields predictions over possible interactions or no-interactions at the last layer.  

\partitle{HO-RCNN~\cite{chao2018learning}.} HO-RCNN is a three-stream Convolutional Neural Network. Each stream considers the appearance of either the human, the object or the human-object (pairwise). Human and object streams consider the global appearance of human and object regions obtained via Region-of-Interest pooling~\cite{fastrcnn}, whereas pairwise stream considers the spatial layout of human-object locations. Spatial locations are critical especially to identify a possible interaction between a human and an object. The detector is built upon the Faster-RCNN backbone~\cite{faster-rcnn}. For human-object detection, the model makes use of this backbone pre-trained on MS-coco~\cite{mscoco}. HOI recognition is achieved by combining the individual predictions of the three streams. 

\partitle{iCAN~\cite{gao2018ican}.} iCAN follows the same network structure as HO-RCNN, and couples HO-RCNN network with a self-attention mechanism~\cite{nonlocal} called instance-centric attention layer for the human and the object streams. This highlights the fine-grained details within human-object regions that are essential to HOIs.  

\partitle{TIN~\cite{li2019transferable}.} TIN augments iCAN with an interactivity classifier, that predicts whether if a given pair of human-object are in interaction or not. The authors prune (suppress) those pairs that are predicted to be non-interacting by the interactivity classifier prior to recognition. Since it is critical to identify which pairs are interacting before the recognition, the authors obtain a considerable improvement in both rare and nonrare interactions over iCAN.  

\partitle{Implementation details.} All the models are trained for $1.8$ million iterations with image-based training~\cite{faster-rcnn}. The learning rate is set to $0.001$ decayed after $900k$ iterations. Weight decay ($0.0001$), dropout (with keep probability $p=0.4$) and batch normalization~\cite{batchnorm} is used for regularization. We include all human detections with a confidence higher than $0.8$ and all object detections with a confidence higher than $0.3$. Using this standard gave a boost to HO-RCNN as it yields better results than iCAN in our experiments. 

%We train all the models for $X$ amount of iterations, using SGD with learning rate $X$ decayed by a factor $X$ after $X$ epochs. 

%\subsection{Diagnostic Method}

%We diagnose the HOI detection in three steps, namely Human-object detection, Human-object interaction identification and Human-object interaction recognition. For each step, we investigate the possible performance gap between rare and nonrare interaction categories. Then, we focus on the source of the specific step. 

%\partitle{Detection of Human and Object.} To diagnose human and object detection, we measure the recall of the off-the-shelf detector Faster-RCNN commonly used by all three models, for humans and objects available in the image. We first measure the recall for the full dataset, for the rare categories and for the nonrare categories. Then, we study the sensitivity of the detector to the human and object pixel size and occlusion. We measure area as... We measure occlusion as 

%\partitle{Identification of Human-Object Interaction.} To diagnose HOI Identification, we measure the binary accuracy of identification performance for each models. Only TIN~\cite{X} provides such prediction. To obtain interacion-no interaction scores from each models, we obtain maximum response over interaction and non-interaction predictions from each model. After obtaining the identification performance, we then study the effect of human-object distance and human-object clutter in identification performance. We compute human-object distance as... We compute human-object clutter as...

%\partitle{Recognition of Human-Object Interaction.} To diagnose HOI recognition, we measure the class-level mean Average Precision (mAP) of recognition performance as is the best practice~\cite{X}. Then, we study the effect of detection and identification errors in recognition performance. 


%The goal of a HOI detector is to determine all possible Human-object interactions from the input image in terms of \texttt{<subject, predicate, object>} triplets. In this work we experiment with $4$ HOI detectors, namely HO-RCNN~\cite{X}, iCAN~\cite{X}, TIN~\cite{X} and NoFrills~\cite{X}. 
%We choose these detectors due to their state-of-the-art performance, and available code online~\footnote{X}. Here we give a brief overview of the workings of these models. 

%\partitle{Human and object detection.}
%The first step in HOI detection is to detect individual Humans and Objects within the image. The models outsource this step to an off-the-shelf object detector named Faster-RCNN~\cite{X}. Faster-RCNN is trained on the large-scale MS-coco dataset for detecting $80$ different object categories common with the HOI detection benchmark~\cite{X}. The object detector returns a big set of Human-object detections per image. Then, the authors set a pre-defined confidence threshold ($0.3$ for objects and $0.8$ for humans) to select only high confidence human and object detections for further processing. 

%\partitle{HOI identification.} 
%The second step in HOI detection is to identify which pair(s) of human-objects are interacting. To achieve this, the models first pair each detected humans and objects. Then, these regions are processed via a three-stream CNN of Human-stream, Object-stream and Pairwise-stream. Pairwise-stream either models only spatial layout of human-object bounding boxes~\cite{X,X} or also human pose~\cite{X,X}. The goal of pairwise stream is to inform the classifier about the relative location of humans and objects therefore making it easier to identify the interaction. The models treat this as a classification task where the given human-object is either assigned to \textit{interaction} or \textit{no-interaction} category. Pair(s) that are assigned to interaction category will further be used to classify the type of the interaction. 

%\partitle{HOI recognition.} 
%The third and last step in HOI detection is the classification of the interaction. Given an interacting pair, the models need to assign the pair to appropriate interaction classes that are represented by \texttt{<verb, noun>} tuples, such as \texttt{<ride, bicycle>} or \texttt{<eat, cake>}. This step is implemented with an N-way classifier that considers the human appearance, object appearance and pairwise appearance to arrive to assign the correct interactions for the input region. Since potentially a human-object can do multiple simultaneous interactions (\ie \texttt{<ride, bicycle>} and \texttt{<hold, bicycle>}), sigmoid non-linearity is applied on top of classifier response before computing the cross entropy. 

%\partitle{Implementation details.}


%\subsection{Diagnostic Methodology}

%\subsubsection{Human-object Detection}

%To diagnose Human and object detection step, we study the relation of detector confidence with respect to the human and the object area and occlusion. 

%We compute the normalized area of a ground truth human or object region by multiplying the width and height of the region divided by the number of pixels within the image. This gives us the ratio of pixels occupied by the specific human or object region. Given human-object detections, we compute the Intersection-over-Union (IoU) between each detections and the ground truth, and assign the detected region as a success if it has an overlap over $0.50$ as is the best practice with PASCAL VOC~\cite{X}. 

%To measure the amount of occlusion over human by the object area or vice versa, we develop an IoU-like metric. To compute object occlusion on human region, we divide the intersection of human-object by the object area. Similarly to compute the human occlusion on object region, we divide the intersection of human-object by the human area. 

%\subsubsection{HOI Identification}

%To diagnose HOI identification, we study the relation of identification confidence with respect to human-object area and the background clutter. 

%To compute the likelihood of interaction, we take the maximum response over all possible interaction categories. The intuition is that if the model can successfully distinguish interacting human-object pairs from non-interacting ones, then the maximum response for a physical interaction category has to be small. 

%We compute the area of human-object region similar to above. However, this time we compute the area of the union of human-object region rather than individually.

%We compute the amount of clutter by counting the number of human and object detectors that do not have a sufficient overlap with any ground truth human-objects (\ie \textless $0.50$). This gives us a measure of how many non-interacting human-object pairs are in the image. More pairs are likely to challenge identification performance. 

%\subsection{HOI Recognition}

%To diagnose HOI recognition, we study the relation of recognition performance with respect to human-object area, human-object clutter, Human-object detection, HOI Identification and HOI population.  

%We compute human-object area and clutter the same way as above. For human-object detection, we assume oracle detection performance where all the humans and objects are recalled. For human-object identification, we assume oracle identification performance where all possible human-object interacters are identified. To measure the relation between HOI population and recognition, we count the number of training instances for each interaction category. 




==> Diagnosing Human-object Interaction Detection/3-experiment.tex <==
\section{Diagnostic Analysis}

We diagnose the HOI detection in three steps, namely Human-object detection, HOI identification, and HOI recognition. We use the standard rare/nonrare split proposed in~\cite{chao2018learning}. 

\subsection{Detection of Human and Object}

To diagnose human and object detection, we first measure the recall of the off-the-shelf detector Faster-RCNN~\cite{faster-rcnn} commonly used by all three models. We measure the recall using the traditional PASCAL VOC criteria~\cite{pascalvoc} that Intersection-over-Union IoU $\textgreater 0.50$  over the full, the rare and the nonrare splits. Results can be seen from Table~\ref{tab:exp11}.

\begin{table}[h]

\begin{center}
%\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{8.5pt}
%\begin{sc}
%\begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{lccccc}

\toprule
   & Full & NonRare & Rare \\
\midrule 

Human  & $86$ & $86$ & $92$ \\ 
Object & $63$ & $64$ & $90$ \\ 
\midrule 

\end{tabular}
%\end{adjustbox}
%\end{sc}
   \caption{Recall of human and object detections.}
\label{tab:exp11}
\end{center}
\end{table}

%Results indicate that there is no gap in terms of localization of humans and objects between rare and nonrare interaction categories. Indeed, the recall of humans and objects from rare interactions is consistently higher than nonrare counterpart. It can also be seen that human localization is easier than object localization. 

Results show that there is no gap in terms of human and object detection performance between rare and nonrare categories. This indicates that recognizing rare interactions is not altered by the detection step. 

Then, we study the sensitivity of the detector to the area and the occlusion. We measure the area of a bounding box by the width $\times$ height of the box divided by the number of pixels in the image. We measure the occlusion of box $b_j$ on $b_i$ as $\dfrac{b_{i} \cap b_{i}}{area(b_{j})}$~\cite{vezhnevets2015object}. An area or occlusion is small if $\textless 0.20$. Results can be seen from Table~\ref{tab:exp12}.

\begin{table}[h]

\begin{center}
%\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{6.5pt}
%\begin{sc}
%\begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{lccccc}

\toprule
   & Full     & \multicolumn{2}{c}{Area} & \multicolumn{2}{c}{Occlusion} \\ 
   &  & Small & Bigger & Small & Bigger \\
 \midrule
Human  & $86$ & $44$ & $94$ & $95$ & $66$ \\ 
Object & $63$ & $26$ & $79$ & $84$ & $43$ \\ 
   
\midrule 

\end{tabular}
%\end{adjustbox}
%\end{sc}
   \caption{Sensitivity of human-object detection.}
\label{tab:exp12}
\end{center}

\end{table}

Results indicate that the off-the-shelf detector is sensitive to both the small area and the large occlusion of humans and objects. This can limit the performance in subsequent steps since many human-object interactors occupy a small region in the image and is occluded by each other. We give detection examples in Figure~\ref{fig:detector} for the human and the objects (green for detected, red for missed boxes). Observe how, within the same image, the detector fails to localize the humans or the objects that have bigger occlusions or occupy a small region.   

\begin{figure}[h]
\begin{center}
\includegraphics[width=1.00\linewidth]{figures/exp0detection.pdf}
\end{center}
  \caption{Example human-object detector \textcolor{green}{success} and \textcolor{red}{failure} cases.}
  \label{fig:detector}
\end{figure}

It is concluded that localization of humans and objects is not altered for rare interactions, however, is affected by the area and the occlusion on human and object regions. 



%In this experiment we test the sensitivity of human and object detection to the pixel area, occlusion and background clutter. 

%\begin{figure}[h]
%\begin{center}

%\includegraphics[width=1.0\linewidth]{figures/exp1area.pdf}
%\end{center}

%\caption{Effect of area on the detectability of humans and objects. Off-the-shelf detector performance is affected by the small size humans and objects.}
%\label{fig:exp1area}
%\end{figure}

%\partitle{Sensitivity to area.} In Figure~\ref{fig:exp1area} we plot the confidence of human and object detector against the normalized area of human and object regions. As human detection works better than object detection, there is an overall margin of $0.20$ confidence points between human and object detection confidence. The detector can better identify humans and objects if they occupy more than $20\%$ of the whole image. Below this threshold, both human and object detection is altered drastically. This has a negative consequence on HOI detection since many interacted objects typically have small area. 

%\begin{figure}[h]
%\begin{center}

%\includegraphics[width=1.0\linewidth]{figures/exp1occlusion.pdf}
%\end{center}

%\caption{Effect of occlusion on detectability.}
%\label{fig:exp1occlusion}
%\end{figure}

%\partitle{Sensitivity to occlusion.} In Figure~\ref{fig:exp1occlusion} we plot the confidence of human and object detector against the amount of occlusion. As can be seen, increasing amount of occlusion severely affects the detector confidence for both humans and objects. 


%\partitle{Sensitivity to clutter.} In Figure~\ref{fig:exp1clutter} we plot the confidence of human and object detector against the amount of background clutter. As can be seen, increasing amount of clutter alters human and object detector performance. 

%\partitle{Qualitative analysis.} In Figure~\ref{fig:exp1qualitative} we showcase examples of detector failures. 

\subsection{Identification of Human-Object Interaction}

To diagnose HOI Identification, we measure the binary accuracy of identification (interacting vs. not-interacting) performance. To obtain interaction vs. not-interaction scores from each model, we obtain maximum response over all interaction ($520$ classes) and not-interaction ($80$ classes) categories respectively. Results are in Table~\ref{tab:exp21}. 

\begin{table}[h]

\begin{center}
%\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{8.5pt}
%\begin{sc}
%\begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{lccccc}

\toprule
   & Full & NonRare & Rare \\
\midrule 

HO-RCNN~\cite{chao2018learning} & $79$ & $79$ & $71$ \\

iCAN~\cite{gao2018ican} & $74$ & $75$ & $67$ \\

TIN~\cite{li2019transferable} & $82$ & $82$ & $77$  \\
\midrule 

\end{tabular}
%\end{adjustbox}
%\end{sc}
   \caption{Identification accuracy of human-object interaction for rare and non-rare interaction categories.}
\label{tab:exp21}
\end{center}
\end{table}

Results reveal that for all three models there is a consistent gap in the identification performance between rare and nonrare interactions. This indicates that the models demand more training examples to learn interactivity. 

We then study the sensitivity of human-object distance and human-object clutter in identification accuracy. We compute human-object distance as the number of pixels between the centers of humans and objects divided by the number of pixels in the image. We compute human-object clutter as the number of human-objects in the background (\ie not involved in any interaction). The distance is deemed to be small if $\textless 0.20$ and the clutter deemed to be small if less than $5$ other human-objects exist in the background. Results can be seen from Table~\ref{tab:exp22}.

\begin{table}[h]

\begin{center}
%\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{4.5pt}
%\begin{sc}
%\begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{lccccc}

\toprule
   & Full     & \multicolumn{2}{c}{Distance} & \multicolumn{2}{c}{Clutter} \\ 
   &  & Small & Bigger & Small & Bigger \\
 \midrule
HO-RCNN~\cite{chao2018learning}  & $79$ & $94$ & $77$ & $91$ & $69$ \\ 
iCAN~\cite{gao2018ican}    & $74$ & $91$ & $72$ & $88$ & $65$ \\ 
TIN~\cite{li2019transferable}     & $82$ & $96$ & $80$ & $93$ & $74$ \\ 
      
\midrule 

\end{tabular}
%\end{adjustbox}
%\end{sc}
   \caption{Sensitivity of identification.}
\label{tab:exp22}
\end{center}

\end{table}

%Results indicate that the HOI identification is highly influenced by the human-object distance and human-object clutter. All three models find it hard to judge whether a given human-object pair is interacting once the distance between human-object gets bigger. This indicates that the models leverage spatial location of humans and object to identify the interactors. Another observation is that the models are altered by the existence of background clutter in the image. This is expected since the number of humans and objects in the image increase the amount of exhaustive pairs to be judged for interaction identification. 

Results indicate that HOI identification is challenged by human-object distance. The models tend to assign distant human-objects to not-interaction category, leading to errors in identification. This shows that the models mostly leverage the spatial layout of human and object locations to identify the interaction. 

It is also clear that background objects confuse the HOI identification step. As the number of possible human-object pairs increases with the background human-objects, the classifier finds it hard to distinguish interacting pairs from non-interacting ones. 

\begin{figure}[h]
\begin{center}
\includegraphics[width=1.00\linewidth]{figures/exp1identification.pdf}
\end{center}
  \caption{Failure examples for HOI Identification of TIN~\cite{li2019transferable}. The rider (above) and the surfer (below) is paired with three other surrounding objects even though there is no interaction in between, lowering the identification performance.}
  \label{fig:identification}
\end{figure}

The effect of the human-object distance and the human-object clutter on identification is visualized in Figure~\ref{fig:identification} for TIN~\cite{li2019transferable}. In both images there are multiple humans and multiple objects, making it a real test for HOI identification. The rider (above) and the surfer (below) are paired with three other surrounding objects with even though there is no interaction in between, lowering the identification performance. 

It is concluded that HOI identification is inferior for the rare interaction categories, and HOI identification is altered by the existence of the human-object distance and human-object clutter. 

%In this experiment we test the sensitivity of Human-object interaction identification to the human-object area and human-object clutter in the background. 


%\begin{figure}[h]
%\begin{center}

%\includegraphics[width=1.0\linewidth]{figures/exp2area.pdf}
%\end{center}

%\caption{Effect of area on identifiability.}
%\label{fig:exp2area}
%\end{figure}

%\partitle{Sensitivity to area.} In Figure~\ref{fig:exp2area} we plot the identification performance against the area of the union of human-object.



%\begin{table}[h]

%\begin{center}
%\renewcommand{\arraystretch}{1.5}
%\setlength\tabcolsep{4.5pt}
%\begin{sc}
%\begin{adjustbox}{max width=\textwidth} 
%\begin{tabular}{lccccc}

%\toprule
% Method  & Full & Crowded & NoCrowded & Rare & NonRare \\
%\midrule 

%Random & X & X & X & X & X \\

%HORCNN & $79$ & $69$ & $93$ & X & X \\

%iCAN & $74$ & $65$ & $90$ & X & X \\

%TIN & $82$ & $74$ & $94$ & X & X \\

%NoFrills & X & X & X & X & X\\


%\end{tabular}
%\end{adjustbox}
%\end{sc}
%   \caption{Identification accuracy of existing techniques.}
%\label{tab:exp1}
%\end{center}

%\end{table}


%\partitle{Sensitivity to clutter.} In Figure~\ref{fig:exp2clutter} we plot the identification performance 
%against the number of clutter human-objects in the background. 

%\begin{figure}[h]
%\begin{center}

%\includegraphics[width=1.0\linewidth]{figures/exp2dist.pdf}
%\end{center}

%\caption{Effect of distance on identifiability.}
%\label{fig:exp2distance}
%\end{figure}


%\partitle{Sensitivity to human-object distance.} In Figure~\ref{fig:exp2distance} we plot the identification performance against the normalized distance between human and object bounding boxes.

\subsection{Recognition of Human-Object Interaction}

%In this experiment we test the sensitivity of Human-object interaction recognition performance against the area of human-objects, clutter of human-objects. We also ablate human, object, and spatial stream to understand the contribution of each stream separately for this task. Finally, we measure the sensitivity of recognition to the detection and identification errors. 

%\partitle{Sensitivity to area.} In Figure~\ref{fig:exp3area} we plot the recognition performance against the area of human-object region. 

%\partitle{Sensitivity to clutter.} In Figure~\ref{fig:exp3clutter} we plot the recognition performance against the amount of clutter within the image. 

%\partitle{Performance of human, object and spatial streams.}

%\partitle{Sensitivity to detector errors.}

%\partitle{Sensitivity to identification errors.}


To diagnose HOI recognition, in line with detection and identification steps, we measure the overall performance at the human-object instance-level. Specifically, we compute the mean Average Precision of interaction classification performance, which is then averaged over all pairs (not over classes) over the dataset. The results are presented in Table~\ref{tab:exp31}. 

\begin{table}[h]

\begin{center}
%\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{8.5pt}
%\begin{sc}
%\begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{lccccc}

\toprule
   & Full & NonRare & Rare \\
\midrule 

HO-RCNN~\cite{chao2018learning} & $9$ & $10$ & $1$ \\

iCAN~\cite{gao2018ican} & $8$ & $9$ & $1$ \\

TIN~\cite{li2019transferable} & $10$ & $10$ & $2$  \\
\midrule 

\end{tabular}
%\end{adjustbox}
%\end{sc}
   \caption{Recognition mAP for rare and non-rare interaction categories.}
\label{tab:exp31}
\end{center}
\end{table}

Results are in line with the class-based mAP reported in all three models ~\cite{chao2018learning,gao2018ican,li2019transferable}, as there is a big gap in recognizing rare and nonrare interaction instances. We then measure the sensitivity of recognition to the detection and identification errors. A detection is correct if IoU $\textgreater 0.50$, and incorrect otherwise. An identification is correct if the accuracy is $1$. Results can be seen from Table~\ref{tab:exp32}.

\begin{table}[h]

\begin{center}
%\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{3.5pt}
%\begin{sc}
%\begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{lccccc}

\toprule
   & Full     & \multicolumn{2}{c}{Detection} & \multicolumn{2}{c}{Identification} \\ 
   &  & Incorrect & Correct & Incorrect & Correct \\
 \midrule
HO-RCNN~\cite{chao2018learning}  & $9$ & $3$ & $14$ & $3$ & $16$ \\ 
iCAN~\cite{gao2018ican}    & $8$ & $3$ & $13$ & $4$ & $13$ \\ 
TIN~\cite{li2019transferable}     & $10$ & $4$ & $14$ & $4$ & $23$ \\ 
\midrule 

\end{tabular}
%\end{adjustbox}
%\end{sc}
   \caption{Sensitivity of recognition.}
\label{tab:exp32}
\end{center}

\end{table}

Results indicate that both the detection and identification errors alter the recognition performance as expected. However, a correct detection or identification does not guarantee perfect recognition accuracy, indicating that the human-object representation is not discriminative. 

==> Diagnosing Human-object Interaction Detection/4-conclusion.tex <==
\section{Conclusion}


%In this paper we focused on rarity in HOI detection. We first investigated the detection step, and find that the detection is altered by the area and the occlusion. This calls for interaction-specific human-object detectors, since for a conventional object detector occlusion is a nuisance whereas in HOIs it hints through the interaction. Human-objects form unique types of occlusions due to interaction-specific body deformations.

This paper focused on rarity in HOI detection in three steps. We revealed that human-object detection is altered by occlusions and area, that are abundant in HOIs. This calls for interaction-specific human-object detectors since for a conventional detector occlusion is a nuisance rather than a signal. We also showed that identifying rare HOIs is difficult which calls for finer-grained reasoning beyond spatial layout. Lastly, we show that recognition is limited by detection and identification errors, which leaves a big room for improvement for these specific steps. 

==> Diagnosing Human-object Interaction Detection/style.tex <==

% include packages
\usepackage{cvpr}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{caption}
\usepackage[nocompress]{cite}
\usepackage{slashbox}
\usepackage[dvipsnames,table]{xcolor} % loads also »colortbl«
\usepackage[toc,page]{appendix}
\usepackage{enumerate}% http://ctan.org/pkg/enumerate
\usepackage{tabularx,ragged2e}
\usepackage{spreadtab}
\usepackage{adjustbox}
\usepackage{booktabs}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{color, colortbl}
%\usepackage{subcaption}
\usepackage{subfigure}

\usepackage[inline]{enumitem}


% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

% space between table and caption caption
\captionsetup[table]{skip=8pt}

% graphics path
\graphicspath{{./figures/}}

% every instance of \includegraphics
\DeclareGraphicsExtensions{.jpeg,.png,.eps,.pdf}

\definecolor{Gray}{gray}{0.9}
\newcommand{\mc}[2]{\multicolumn{#1}{c}{#2}}
\definecolor{Gray}{gray}{0.85}
\definecolor{LightCyan}{rgb}{0.88,1,1}

\newcolumntype{a}{>{\columncolor{Gray}}c}
\newcolumntype{b}{>{\columncolor{white}}c}

\newcommand{\str}[1]{\textcolor{ForestGreen}{[\textbf{STR}: #1]}}
\newcommand{\Arnold}[1]{\textcolor{Red}{[\textbf{AS}: #1]}}
\newcommand{\arnold}[1]{\textcolor{Red}{[\textbf{AS}: #1]}}
\newcommand{\mert}[1]{\textcolor{Blue}{[\textbf{MK}: #1]}}
\newcommand{\parspace}{\bigbreak}
\newcommand{\ptspace}{\vspace*{5pt}}
\newcommand{\partitle}[1]{\bigbreak\noindent\textbf{#1}}
\newcommand{\addref}{\textcolor{red}{[\textbf{REF}]\xspace}}
\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argminA}{arg\,min} % Jan Hlavacek
\DeclareMathOperator*{\argminB}{argmin}   % Jan Hlavacek
\DeclareMathOperator*{\argminC}{\arg\min}   % rbp

\newcommand{\argminD}{\arg\!\min} % AlfC
%\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}

\newcommand{\argminE}{\mathop{\mathrm{argmin}}}          % ASdeL
\newcommand{\argminF}{\mathop{\mathrm{argmin}}\limits}   % ASdeL
\newcommand{\Ree}{\mathbb{R}}

\newcommand{\dummyfig}[1]{
  \centering
  \fbox{
    \begin{minipage}[c][0.25\textheight][c]{0.45\textwidth}
      \centering{#1}
    \end{minipage}
  }
}


% COMMENTING COMMANDS

%\newcommand{\etal}{\textit{et al}. }
%\newcommand{\ie}{\textit{i}.\textit{e}., }
%\newcommand{\eg}{\textit{e}.\textit{g}. }

% limits on side
\DeclareMathOperator{\argminG}{arg\,min} % Jan Hlavacek
\DeclareMathOperator{\argminH}{argmin}   % Jan Hlavacek
\newcommand{\argminI}{\mathop{\mathrm{argmin}}\nolimits} % ASdeL

\cvprfinalcopy % *** Uncomment this line for the final submission

\def\cvprPaperID{3} % *** Enter the CVPR Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% Pages are numbered in submission mode, and unnumbered in camera-ready
%\ifcvprfinal\pagestyle{empty}\fi
